Escaping the One-Step Trap: Temporal Shortcuts and Stopped-Option Semigroups for Jumpy World Models

Standard world models simulate the future one primitive action at a time, spending fixed test-time compute on short-term physics rather than long-horizon decisions. Jumpy world models escape this one-step trap by predicting an option's multi-step outcome in $O(1)$ evaluations, unifying denoising shortcuts with option-semigroup composition across physical time. We formalize this as a five-tuple stopped-option semigroup separating skill stopping from episode termination, conditioning readouts jointly on the realized endpoint, and composing jumps ($h + h \to 2h$). Across 319 models and 770,000+ episodes over eight model families, four control tasks, and five latent geometries, we establish four principles for jumpy planning. (1) Shortcuts amplify subgoal reachability rather than jump length: planning fails on non-covering skills (0% on PinPad and Sokoban) and gains >41 points as subgoals unlock at fixed ~56-step durations. (2) Endpoints dictate discounting: marginal duration and return heads blur fast arrivals with slow timeouts, inflating option-Bellman error up to $23.5\times$ and losing 29.3 points on risky shortcuts. (3) Bounded norms hide a manifold trap: on convex simplices, two-step flows drift into an unsupervised interior, amplifying dyadic return drift to $4.85\times 10^8$; endpoint anchoring and spherical geodesics prevent divergence across all 27/27 full-budget runs. (4) On full-span near-deterministic data, single-step anchored expectation reaches 54.75% solve rate at 256 evaluations -- beating multi-step flows at $16\times$ compute -- while option commitment cuts episode compute $25.5$-$27.2\times$; under truncated spans ($h \le 16$) or bimodal noise, spherical semigroup flows hit the lowest $8\times$ extrapolation error (0.193) and gain $+10.2$ points via multi-particle planning.

==> fonts/arial-setup.tex <==
\pdfmapfile{+fonts/arial.map}
\DeclareFontFamily{T1}{labarial}{}
\DeclareFontShape{T1}{labarial}{m}{n}{<-> fonts/arialregular}{}
\DeclareFontShape{T1}{labarial}{m}{it}{<-> fonts/arialitalic}{}
\DeclareFontShape{T1}{labarial}{m}{sl}{<-> fonts/arialitalic}{}
\DeclareFontShape{T1}{labarial}{b}{n}{<-> fonts/arialbold}{}
\DeclareFontShape{T1}{labarial}{bx}{n}{<-> fonts/arialbold}{}
\DeclareFontShape{T1}{labarial}{b}{it}{<-> fonts/arialbolditalic}{}
\DeclareFontShape{T1}{labarial}{bx}{it}{<-> fonts/arialbolditalic}{}

